Do Visual Imaginations Improve Vision-and-Language Navigation Agents?

Vision-and-Language Navigation (VLN) agents are tasked with navigating an unseen environment using natural language instructions. In this work, we study if visual representations of sub-goals implied by the instructions can serve as navigational cues and lead to increased navigation performance. To synthesize these visual representations or imaginations, we leverage a text-to-image diffusion model on landmark references contained in segmented instructions. These imaginations are provided to VLN agents as an added modality to act as landmark cues and an auxiliary loss is added to explicitly encourage relating these with their corresponding referring expressions. Our findings reveal an increase in success rate (SR) of around 1 point and up to 0.5 points in success scaled by inverse path length (SPL) across agents. These results suggest that the proposed approach reinforces visual understanding compared to relying on language instructions alone. Code and data for our work can be found at https://www.akhilperincherry.com/VLN-Imagine-website/.

==> tables/no_loss_cosine.tex <==
\begin{table}
	\centering
	\tabcolsep=0.30cm
	\caption{Sequential \vs goal imagination; HAMT-Imagine. We study the effect of providing the HAMT-Imagine agent with just the imagination belonging to the final valid sub-instruction relative to full valid imaginations. We observe providing just the goal imagination improves performance significantly compared to baseline but shows lower performance relative to providing the agent with full imaginations.}
	\label{tab:no_loss_ablation}
	\begin{tabular}{p{4.5cm} cc} \toprule
		& SR$\uparrow$ & SPL$\uparrow$ \\\midrule
  		Baseline (HAMT) & 66.24 & 61.51 \\ 
            HAMT-Imagine + $\mathcal{L}_{cos}$ & 67.26 & 62.02 \\ 
            HAMT-Imagine - loss & 66.75 & 61.6 \\ \bottomrule
	\end{tabular}
\end{table}
